On the Centralization and Regionalization of the Web

Over the past decade, Internet centralization and its implications for both people and the resilience of the Internet has become a topic of active debate. While the networking community informally agrees on the definition of centralization, we lack a formal metric for quantifying centralization, which limits research beyond descriptive analysis. In this work, we introduce a statistical measure for Internet centralization, which we use to better understand how the web is centralized across four layers of web infrastructure (hosting providers, DNS infrastructure, TLDs, and certificate authorities) in 150~countries. Our work uncovers significant geographical variation, as well as a complex interplay between centralization and sociopolitically driven regionalization. We hope that our work can serve as the foundation for more nuanced analysis to inform this important debate.

==> acks.tex <==
Deepak Kumar
Phillip Stephens

==> clustering.tex <==
\section{Clustering Providers}
\label{sec:clustering}

\paragraph{Clustering hosting providers} We use hosting providers' usage and
endemicity ratio to cluster providers with similar geographic popularity
characteristics. First, we threshold out providers that sit in the long tail:
those that do not host at least 0.1\% of websites in any country or that have a
total usage less than 10. This
separates \TK long-tail providers from \TK others. Next, we notice that high
usage and low endemicity ratio are loosely correlated, but with a meaningful
signal in how data points deviate from that correlation; thus, to isolate this
signal, 
we use principal component analysis (PCA) to transform the usage vs.
endemicity ratio data along the axes of highest variance. 

From there, we normalize the data using min-max scaling and cluster the
providers using affinity propagation.

\footnote{Affinity propagation is a nonparametric clustering technique that does
not require specifying the number of clusters and can handle varying-density
clusters. It operates by sending messages between data points until convergence}

%https://scikit-learn.org/stable/modules/clustering.html#affinity-propagation
% This results in 17 clusters, shown in Figure~\ref{fig:hosting_clusters}.


==> regionalization_ca.tex <==
\subsection{Regional Clusters}

\subsubsection{Overall}
The most popular countries for providing certificates are USA, UK, and Belgium (82.7\%, 11.3\%, 4.7\% of all sites, respectively).

\subsection{Country-wise}
\subsubsection{USA}
There are 9 CAs headquartered in USA that provide certificates to the sites in our dataset. The most popularly used ones include DigiCert, Internet Security Research Group (Let's Encrypt), and Google (31.9\%, 21.9\%, 12.4\%, 6.0\% of the sites in our dataset use these as their CA). If we remove duplicate sites, we see Let's Encrypt dominates with 37.9\% of the sites using it.

\subsubsection{UK}
The only CA we found in our dataset that is headquartered in the UK was Sectigo, which made up 11.3\% of the total CA usage.

\subsubsection{Belgium}
GlobalSign, which is headquartered in Belgium, makes up 4.7\% of the total CA usage in our dataset. Although GlobalSign has a global penetration, only 10.5\% of the sites in the Belgium top list use it. US-based CAs and Sectigo (UK) make up 73.3\% and 15.6\% of the CA usage in Belgium.

\subsubsection{Poland}
We note that Iran and Afghanistan have a significant proportion of sites that have certificates provided by Polish CAs (19.6\% and 5.4\% respectively). Interestingly, when compared to Iran, fewer Polish sites rely on Polish CAs (18.9\%). 

\subsubsection{Insularity}
Several countries rely strongly on the CAs headquartered within them. For example, the 5 most insular countries (when it comes to CAs) include the US (86.0\%), Poland (18.9\%), Taiwan (16.4\%), Japan (14.4\%), UK (11.5\%). While the CAs in the US and UK are used globally, the rest of these countries have CAs that are largely regional.

==> regionalization_providers.tex <==
\subsection{Regional Clusters}
In this section, we detail patterns and regional clusters formed when we observed the hosting provider usage in the top 10k sites in 150 countries.

\subsubsection{USA} 
Hosting is dominated by US-based providers. We note that all countries have at least one
site in their top list hosted in the US. 67.7\% or 53.0\% of all top visited sites (across 150
countries) are hosted in the US if we include or exclude duplicates,
respectively. 
Cloudflare is the most dominant provider, with 35.0\% of the sites in our dataset (24.2\% if we exclude duplicates) hosted in it. In the US, the next most popular hosting providers are Amazon, Akamai, and Google (they make up 10.1\%, 3.9\%, and 3.8\% of the total usage). If we consider individual top sites lists of countries, USA is the
country where the highest percentage of top sites are hosted for all countries
except 5 (Belarus, Czechia, Hungary, Iran, and Russia). In these 5 countries, they themselves host most of their content. 

\subsubsection{Russia} For all of the former USSR countries \footnote{Former
USSR countries include Armenia, Azerbaijan, Belarus, Estonia, Georgia,
Kyrgyzstan, Kazakhstan, Latvia, Moldova, Russia, Tajikistan, Turkmenistan,
Uzbekistan, Ukraine} (save for Ukraine), a significant portion of their top sites
are hosted in Russia (33.9\% in Turkmenistan to 5.4\% in Estonia). We believe
this is due to economic and political ties (which would also explain why
Ukranian sites tend not to be hosted here). The most popular Russian provider is
Selectel, which makes up 10.8\% of all Russian provider usage.

\subsubsection{Iran} A significant number of sites in the Afghanistan top site
list are hosted in Iran (20.5\%). This could be due to their shared language
(Persian), which would result in frequent usage of Iranian sites in Afghanistan.
Indeed, we note that 31.4\% of the sites in the Afghanistan list are in
Persian\footnote{We detected the language on the site by scraping the text on
the landing page and using the Python library LangDetect \cite{langdetect}.
Sites that crashed were excluded.}, of which 60.8\% are hosted in Iran.

\subsubsection{France} Hosts the second highest number of total origins (4.5\%
or 4.3\% with or without duplicates, respectively). OVH is based here, which
accounts for 70.7\% of all French provider usage. 3 French administrative
regions (Réunion Island, Guadeloupe, and Martinique) host a significant number of
sites here (35.6\%, 34.3\%, 35.1\%). When compared to these administrative
regions, France has fewer percentage sites hosted by itself (31.8\%). We also note several African countries host a lot of their content in France e.g. Burkina Faso (21.1\%), Côte d'Ivoire (18.1\%), Mali (18.0\%). This could be explained through colonial ties.

\subsubsection{Netherlands} Akamai Netherlands is based there, which explains its
global presence as a provider (4.0\% of all top sites, including duplicates).

\subsubsection{Germany} Hetsner is based there, so it has a global presence as a
provider (4.0\% of all top sites, including duplicates).

\subsubsection{Czechia} 25.7\% of the Slovakian top sites are hosted in Czechia.
This could be due to their political history; they were one country before
their separation in 1992. Czechia itself is quite insular and we do not see the
same dependence towards Slovakia.

\subsubsection{Cyprus} Hostinger has a global presence, with 0.5\% of all sites
in our dataset hosted by it. The sites hosted here are not endemic to specific regions. 

==> regionalization_tld.tex <==
\subsection{Regional Clusters}
We analysed the trends in top level domains (TLDs) of sites accessed most
frequently by users in different countries. Many of these TLDs were ccTLDs
(country code TLDs). For example, the TLDs '.us', '.uk', and '.ir' are reserved
for sites managed in the US, UK, and Iran respectively. There also exist
'global' TLDs such as '.com' and '.net'. These TLDs do not have country-specific
requirements.

\subsubsection{Global}
\rumi{Some of this might also be relevant in Insularity.}
The sites in our dataset mostly have global TLDs (68.0\%). For most countries, global TLDs are the most prevalent -- this is not the case for 17 countries \footnote{Brazil, Czechia, Denmark, Estonia, Finland, Greece, Hungary, Italy, Japan, Lithuania, the Netherlands, Norway, Poland, Romania, Russia, Sweden, Slovakia}. For each of these countries, there are more sites with their own associated ccTLDs. This implies that, in these regions, people access their native sites more frequently than 'global' sites.

\subsubsection{Russia}
We see a regional pattern when it comes to the usage of Russian domains. Russian TLDs are also the second most popular category of TLDs (after global ones), with 2.3\% of the sites in our dataset ending with '.ru'. This usage is particularly prominent in former USSR countries, with 36.0\% of Turkmenistan's top sites, to 5.6\% of Ukraine's top sites ending with '.ru'. Interestingly, we also note that for 5 countries (Kyrgyzstan, Latvia, Syria, Tajikistan, Turkmenistan, and Yemen), Russian domains are more popular than their native domains. For all these countries, save Latvia, the '.ru' TLD is the most popular ccTLD.

\subsubsection{France}
The '.fr' ccTLD is the third most popular category of TLDs (2.1\% of all sites). In 14 countries\footnote{Burkina Faso, Benin, Congo, Côte d'Ivoire, Cameroon, Algeria, Guadeloupe, Haiti, Madagascar, Mali, Martinique, Réunion, Senegal, Togo}, French domains are more popular than their own native domains. 3 of these can be attributed to cultural and political similarities as they are French administrative regions (Martinique, Réunion and Guadeloupe). The rest of these countries (with 10 of them being African countries) were once French colonies, and can also be thus explained through cultural and historical significance. 

\subsubsection{Germany}
\rumi{There could potentially be a subsubsection on countries with shared languages because that's a pattern i've noted for several regions e.g germany, iran, spain, brazil}
Several countries where German is a dominant language have a large percentage of sites with a German TLD. These include Germany (44.0\%), Austria (14.1\%), Luxembourg (8.0\%), and Switzerland (7.4\%). 

\subsubsection{Spain}
We also note '.es' ccTLDs are most often used in countries where Spanish is an official language. These include Spain (27.3\%), Cuba (5.6\%), Venezuela (3.9\%), Bolivia (3.8\%), and Nicaragua (3.8\%). In the case of two Spanish-speaking countries (Cuba and Puerto Rico), the '.es' ccTLD is more popular than their native ccTLDs ('.cu' and '.pr').

\subsubsection{Insularity}
The 5 most insular countries are Czechia (66.6\%), Hungary (63.0\%), Poland (62.1\%), Slovakia (58.6\%), and Greece (57.7\%). The 5 least insular countries are Guadeloupe (0.58\%), Martinique (0.64\%), Mali (0.71\%), Yemen (0.85\%), USA (0.87\%).
